Recent Advances in Direct Speech-to-text Translation

Recently, speech-to-text translation has attracted more and more attention and many studies have emerged rapidly. In this paper, we present a comprehensive survey on direct speech translation aiming to summarize the current state-of-the-art techniques. First, we categorize the existing research work into three directions based on the main challenges -- modeling burden, data scarcity, and application issues. To tackle the problem of modeling burden, two main structures have been proposed, encoder-decoder framework (Transformer and the variants) and multitask frameworks. For the challenge of data scarcity, recent work resorts to many sophisticated techniques, such as data augmentation, pre-training, knowledge distillation, and multilingual modeling. We analyze and summarize the application issues, which include real-time, segmentation, named entity, gender bias, and code-switching. Finally, we discuss some promising directions for future work.

==> figures/overview.tex <==
\begin{figure*}[th]
  \centering
\begin{forest}
  forked edges,
  for tree={
    grow=east,
    reversed=true, % if true, in the clockwise direction
    anchor=base west,
    parent anchor=east,
    child anchor=west,
    base=left,
    font=\footnotesize,
    rectangle,
    draw=hiddendraw,
    rounded corners, 
    align=left,
    minimum width=2.5em,
    minimum height=1.2em,
     % edge+={darkgray, line width=1pt},
     % l sep+=2.5pt,
     % s sep+=-5pt,
    s sep=6pt,
    inner xsep=3pt,
    inner ysep=1pt,
  },
  % before packing={where n children=3{calign child=2, calign=child edge}{}},
  % before typesetting nodes={where content={}{coordinate}{}},
  % where level<=1{line width=2pt}{line width=1pt},
  where level=1{text width=8em}{},
  where level=2{text width=11em}{},
  where level=3{font=\scriptsize}{},
  where level=4{font=\scriptsize}{},
  where level=5{font=\scriptsize}{},
  [Overview
    [Main Challenges
    [Modeling Burden]
    [Data Scarcity]
    ]
    [Modeling
      [Encoder-Decoder
        [Bi-LSTM~\cite{Berard_arxiv2016,Weiss_ISCA2017}]
        [Speech-Transformer~\cite{Gangi_NAACL2019,Inaguma_ACL2020}]
        [Conformer~\cite{Gulati_ISCA2020,Wang_AACL2020}]
      ]
      [Decoupled Encoder
        [Supervised Decoupling~\cite{Liu_corr2020,dong2021listen,Xu_ACL2021}]
        [Unsupervised Decoupling~\cite{Wu_ISCA2020,nguyen2022improving,wang2021large}]
      ]
      [Two-Stream Encoder
        [Speech Encoder~\cite{Ye_interspeech2021}]
        [Text Encoder~\cite{tang2021general}]
        [Interaction~\cite{tang2021improving,han2021learning,Ye_NAACL2022}]
      ]
      [Decoupled Decoder
        [Two-pass Decoder]
        [Dual Decoder]
      ]
    ]
    [Training Strategy
      [Data augmentation
        [Expanding ASR or MT data
        % \\\qquad\cite{Pino_ISCA2020,Gaido_IWSLT2020,jia2019leveraging,Pino_corr2019}
        ]
        [Speech Augmentation
% ~\cite{park2020specaugment,mccarthy2020skinaugment}\\\qquad\cite{tsiamas2022segaugment,lam2022make,lam2022sample}
]
      ]
      [Pre-training
        [ ]
        [ ]
      ]
      [Multi-task learning]
      [Knowledge Distillation]
    ]
    % [Inference
    %   [Simultaneous ST
    %     [Metrics]
    %     [Quality-Latency Trade-offs]
    %     [Adaptive Segmentation]
    %   ]
    %   [Speech-to-speech Translation
    %     [Model Structure]
    %     [Pseudo Labeling]
    %     [Metrics]
    %   ]
    %   [Multi-lingual ST]
    %   [Non-autoregressive ST]
    %  ]
     [Application Issues
     [
     Real-time
     ]
      [Segmentation
      ]
      [Named Entity
      ]
      [Gender Bias]
      [Code Switching]
     ]
    ]
\end{forest}
\caption{Overview.}
\label{fig:taxonomy_of_training_design}
\end{figure*}

% [
%      Applications
%      [Segmentation]
%      [Named Entity]
%      [Gender Bias]
%      [Code Switching]
%      ]

==> figures/overview2.tex <==
\begin{figure*}[th]
  \centering
\begin{forest}
  forked edges,
  for tree={
    grow=east,
    reversed=true, % if true, in the clockwise direction
    anchor=base west,
    parent anchor=east,
    child anchor=west,
    base=left,
    font=\footnotesize,
    rectangle,
    draw=hiddendraw,
    rounded corners, 
    align=left,
    minimum width=2.5em,
    minimum height=1.2em,
     % edge+={darkgray, line width=1pt},
     % l sep+=2.5pt,
     % s sep+=-5pt,
    s sep=6pt,
    inner xsep=3pt,
    inner ysep=1pt,
  },
  % before packing={where n children=3{calign child=2, calign=child edge}{}},
  % before typesetting nodes={where content={}{coordinate}{}},
  % where level<=1{line width=2pt}{line width=1pt},
  where level=1{text width=8em}{},
  where level=2{text width=11em}{},
  where level=3{font=\scriptsize}{},
  where level=4{font=\scriptsize}{},
  where level=5{font=\scriptsize}{},
  [Challenges
    [Data Scarcity
        [Data augmentation]
        [Knowledge Distillation]
        % [Pre-training]
        [Transfer learning]
        [Multilingual Training]
    ]
    
    [Modeling
      [Encoder-Decoder
        [Bi-LSTM]
        [Speech-Transformer]
        [Conformer]
      ]
      [Multi-task Framework
         [Decoupled Encoder
            [Supervised Decoupling]
            [Unsupervised Decoupling]
         ]
        [Two-Stream Encoder
            [Speech Encoder]
            [Text Encoder]
            [Interaction]
        ]
          [Decoupled Decoder
            [Two-pass Decoder]
            [Dual Decoder]
          ]
       ]
    ]
   
    [Application Issues
     [
     Real-time
     ]
      [Segmentation
      ]
      [Named Entity
      ]
      [Gender Bias]
      [Code Switching]
     ]
    ]
\end{forest}
\caption{Overview.}
\label{fig:taxonomy_of_training_design2}
\end{figure*}

% [
%      Applications
%      [Segmentation]
%      [Named Entity]
%      [Gender Bias]
%      [Code Switching]
%      ]

==> figures/overview4.tex <==
\begin{figure*}[th]
  \centering
\begin{forest}
  forked edges,
  for tree={
    grow=east,
    reversed=true, % if true, in the clockwise direction
    anchor=base west,
    parent anchor=east,
    child anchor=west,
    base=left,
    font=\footnotesize,
    rectangle,
    draw=hiddendraw,
    rounded corners, 
    align=left,
    minimum width=2.5em,
    minimum height=1.2em,
     % edge+={darkgray, line width=1pt},
     % l sep+=2.5pt,
     % s sep+=-5pt,
    s sep=6pt,
    inner xsep=3pt,
    inner ysep=1pt,
    node options={align=center,},
    text width=2.7cm,
  },
  % before packing={where n children=3{calign child=2, calign=child edge}{}},
  % before typesetting nodes={where content={}{coordinate}{}},
  % where level<=1{line width=2pt}{line width=1pt},
  where level=1{text width=10em}{},
  % where level=2{text width=9em, font=\scriptsize}{},
  % where level=3{font=\scriptsize}{},
  % where level=4{font=\scriptsize}{},
  % where level=5{font=\scriptsize}{},
  where level=2{text width=10.8em}{},
  where level=3{text width=10.7em}{},
  where level=4{text width=6.7em}{},
  where level=5{font=\scriptsize}{},
  [Approaches
    % [Challenges]
    [Tackling Modeling Burden, for tree={fill=red!45,template}
      [Transformer and Variants
        % [Bi-LSTM]
        [Speech-Transformer]
        [Conformer]
        [SSL-Transformer]
      ]
      [Multitask Framework
         [Decoupled Encoder]
        [Two-Stream Encoder
            [Speech Encoder]
            [Text Encoder]
            [Interaction]
        ]
          [Decoupled Decoder
            [Two-pass Decoder]
            [Dual Decoder]
          ]
       ]
       [Non-autoregressive Modeling]
    ]
    [Tackling Data Scarcity
        [Data Augmentation
            [Expanding ST Data]
            [Speech Augmentation]
        ]
        [Pre-training
            [Separate Pre-training]
            [Joint Pre-training]
        ]
        [Knowledge Distillation]
        [Multilingual Training]
    ]
    [Tackling Application Issues
     [
     Real-time
     ]
      [Segmentation
      ]
      [Named Entity
      ]
      [Gender Bias]
      [Code-Switching]
     ]
    ]
\end{forest}
\caption{Taxonomy of speech-to-text translation.}
\label{fig:taxonomy_of_training_design2}
\end{figure*}

==> section/020_e2est.tex <==

\section{End-to-end Speech Translation}
\label{sec:e2est}

\subsection{Task Definition }
\label{sec:e2est_task}
End-to-end speech translation directly translates the source language speech $\mathbf{s}$ to the target language text $\mathbf{y}$. Speech translation corpus usually contains source speech, transcription, and translation. The objective training function of ST model $\theta$ is the negative log-likelihood loss:
\xc{add subscript in equ?}
\begin{equation}
    L_{\theta} = \sum -\log p(\mathbf{y}|\mathbf{s};\theta)
\end{equation}



% \subsection{Datasets}
% \label{sec:e2est_data}
% The history of speech translation technology can be traced back hundreds of years, but the rise of end-to-end research is only a few decades.
% % Due to the late start of end-to-end research, the accumulated training data is still relatively scarce, compared to cascaded systems. 
% % As this paradigm becomes more popular, more and more training data are constructed. 
% This section reviews currently available datasets for end-to-end model training, as shown in Table x.

% \input{table/datasets.tex}


\subsection{Basic Modeling}
\label{sec:e2est_basic_model}
The basic model framework of E2E ST is mainly based on the encoder-decoder structure. As shown in Figure~\ref{fig:enc_dec}, the encoder encodes the speech input into a sequence of hidden states, and the decoder outputs the final translation result condition on the hidden states.
The speech input can be the original waveform audio signal, or speech features such as MFCC, log Mel-filter bank~(Fbank), etc.
The decoder is basically autoregressive, with the estimated probability:
% generating each translation token from left to right:
\begin{equation}
    p(\mathbf{y}|\mathbf{s};\theta) = \prod_{t=1}^T p(y_t|\mathbf{y_{<t}}, \mathbf{s}; \theta)
\end{equation}
In the inference stage, we usually apply beam search to generate target sentences.
We will describe some typical encoder-decoder models in Sec.~\ref{sec:model:enc_dec}.

% But the vanilla encoder-decoder model cannot fully solve the E2E ST task, and in Section x we will discuss modeling challenges, as well as introduce more variants of the model structure in Section x.
% There are also a few non-autoregressive ST models, which will be discussed in Section x. 


==> section/030_challenge.tex <==
\subsection{Challenges}
\label{sec:challenges}

Although the end-to-end ST has achieved dramatic progress in recent years, the cascaded systems are still the first choice in industrial scenarios for their superior performance.
For example, the best end-to-end model is still worse than the cascaded counterpart with a performance gap of more than 1 BLEU point in the latest IWSLT campaign \cite{Anastasopoulos_IWSLT2022}.
Two main challenges limit the potential of the E2E model in the practice application: modeling burden and data scarcity. 
\yr{rigid}

% \subsection{Modeling Burden}
\noindent\textbf{Modeling Burden}
\label{sec:challenge:model_burden}
Translating from source speech to target text requires cross-modal and cross-lingual modeling. 
Conventional cascaded systems decouple it into ASR and MT models~\cite{Ney_IEEE1999,Mathias_ICASSP2006}, while direct translation in an E2E manner is non-trivial.
The intractable issue of heavy modeling burden leads to the challenge of poor convergence, often failing to obtain a well-trained model~\cite{Inaguma_ACL2020,Zhang_ICML2022}.

% \subsection{Data Scarcity}
\noindent\textbf{Data Scarcity}
\label{sec:challenge:data}
The E2E model outperforms the cascaded counterpart trained on limited training data \cite{ye2022gigast}.
However, annotated speech-to-translation data is scarce, resulting in that the E2E model is inferior to the cascaded systems trained on abundant ASR and MT data \cite{sperber2020speech}.
From the perspective of large-scale open datasets, the Librispeech dataset in ASR includes 960 hours of speech \cite{Panayotov_ICASSP2015} and the WMT dataset in MT includes 36M sentence pairs, while the MuST-C dataset in ST only includes 400 hours of speech with 230k utterances \cite{Gangi_NAACL2019}.
In industrial scenarios, the gap in data quantity can even reach tens or hundreds of times.

\xc{add something, and introduce figure 1}


% \subsection{Datasets}
% \label{sec:e2est_data}
% The history of speech translation technology can be traced back hundreds of years, but the rise of end-to-end research is only a few decades.
% Due to the late start of end-to-end research, the accumulated training data is still relatively scarce, compared to cascaded systems. 
% As this paradigm becomes more popular, more and more training data are constructed. 
% This section reviews currently available datasets for end-to-end model training, as shown in Table x.



% \yr{costly to make large scale dataset.}
% \yr{Compare ST and MT scale.}
% \yr{Paper that mentioned data scarcity problem}
% \yr{Intro: to}

% \subsection{Online Inference ??}

% \subsection{Advanced Topics (like simul, multilingual...) }

% \subsection{...}

==> section/060_advanced.tex <==
% \section{Advanced Topics}
\section{Inference}
\label{sec:advanced}

\input{section/sist.tex}

% \subsection{Multi-lingual Speech-to-text Translation }
% \subsection{Unsupervised Speech-to-text Translation }



==> section/background_.tex <==
\section{Background }

\subsection{Automatic Speech Recognition}

We describe our starting point in this section, and
provide preliminary context on Transformer-based neural machine translation models.

\subsection{Neural Machine Translation}
In general,  machine translation task is sequence-to-sequence approach which is trained on bilingual language pairs,  using an encoder to encode the source sentence and a decoder to generate the target sequence word by word from left to right. The sentence is split into tokens, which can be words, sub-words
or characters, resulting in pairs of sequences $X=(x_1, x_2,\cdots, x_m)$ and $Y=(y_1, y_2,\cdots, y_n)$, where m and n is the length of the source and the target
sequence respectively. 
The training objective of sequence modeling is usually to  to minimize the negative log-likelihood of the target sequence:
\begin{equation}
      \mathcal{L} = -\sum_{i=1}^{n} \log p_\theta(y_i|y_{<i},X).
      \label{eq:neglike}
\end{equation}
The most common NMT model consists of three modules: an encoder to summarize the source representation , a decoder to generate the target translation and a cross-attention mechanism to bridge the encoder and the decoder.  The encoder and the decoder of NMT can be LSTM, CNN and self-attention. In this work, the model architecture is largely based on the current state-of-the-art Transformer model~\cite{vaswani2017attention}, while it is generally applicable to other types of NMT architectures. 
Specifically, the encoder transfer the input sequence $X$ into a sequence of dense vector of the same length and the decoder $H$. Then, the decoder generate the target sequence $Y$ sequentially based on the source representation $H$. 
\begin{align}
    H &= \text{Encoder}(X)  \\ 
    y_{i} &= \text{Decoder}(H, y_{<i})
\end{align}
Both the encoder and decoder are composed of the same type of blocks, named Transformer blocks. 
Each Transformer block takes a sequence of vectors as input and outputs a sequence
of vectors. 
In the encoder, transformer blocks are composed of two sub-layers, a self-attention
and a feed-forward layer. 
In the decoder, transformer blocks are composed of three sub-layers, a self-attention, an encoder decoder attention
and a feed-forward layer. 
These are applied sequentially and are both followed by a residual
connection and layer normalization. 
The self-attention layer is an attention layer that updates each element of the sequence by
looking at the other elements, while the feed-forward layer (FFN) passes each element of the sequence independently through a 2-layer $1\times1$ convolution network. 

\subsection{Cascaded Speech Translation}

\paragraph{End-to-end Speech Translation} A little different from text translation,  the training corpus for
speech translation contains speech-transcription-translation triples, denoted as $(X,Y,Z)$. 




==> section/e2e_apps_beyond.tex <==
% \section{Applicational Tasks and Beyond} % 还不算Applicational？
\section{Advanced Topics}

along with datasets

\subsection{Simultaneous Speech-to-text Translation}

\subsection{Multi-lingual Speech-to-text Translation}

\subsection{Non-autoregressive Speech-to-text Translation}

\subsection{Unsupervised Speech-to-text Translation}

\subsection{Speech-to-speech Translation}

% \subsection{Advanced Tasks}
% \subsubsection{Disfluent Speech Translation}

% \subsubsection{Gender Problems in Speech Translation}
% MuST-She

% \subsubsection{Context-level Translation}
% ACL's zhangbiao Context help paper.

==> section/e2e_input.tex <==
% \section{Input Representation}

% \subsection{Signal Processing}
% Classic MFCC, FBANK with CNN to shrink length

% \subsection{Pre-trained Audio Representation}
% Wav2vec family

% \subsection{Data Augmentation}

% Leveraging Weakly Supervised Data to Improve End‑to‑End Speech‑to‑Text Translation

% Leveraging Out-of-Task Data for End-to-End AutomaticSpeech Translation

% Harnessing Indirect TrainingData for End-to-EndAutomatic Speech Translation:Tricks of the Trade

% On Using SpecAugment forEnd-to-End SpeechTranslation

% Skinaugment: Auto-EncodingSpeaker Conversions For Automatic speech Translation

% \subsection{Phoneme-aid audio representation}
% \subsubsection{Phoneme compressed}

% \subsubsection{Phoneme fused}

\section{Acoustic and Linguistic Features}

\subsection{Signal Processing}

\subsection{Pre-trained Representation}
\subsubsection{Audio Representation/Text Representation}
% \subsubsection{Text Representation}

\subsection{Linguistic Units}
\subsubsection{IPA/Phoneme/Pinyin/Char/Subword/Word}
% \subsubsection{Char}
% \subsubsection{Subword}
% \subsubsection{Word}

\subsection{Auxiliary Clues}
\subsubsection{Speaker/Rhythm/Accent/Gender/Disfluency/Context aware}
% \subsubsection{Gender-aware}
% \subsubsection{Disfluency-aware}
% \subsubsection{Context-aware}

==> section/e2e_progress.tex <==
\section{How to Solve Data Scarcity? }
\label{sec:data_scarcity}


\subsection{Model design}
\subsubsection{Utilizing Bert-KD, like LUT?}

\subsection{Training strategy}
\subsubsection{Pretraining}

Pre-training is a promising method that first pre-trains different components of the ST on external data, and then fine-tunes the model parameters on the small-scale ST data \cite{Zhuang_IEEE2021}.
The vanilla ST model adopts the encoder-decoder architecture, where a naive strategy initializes the encoder with the ASR model and the decoder with the MT model, and finally fine-tunes all the model parameters \cite{Berard_IEEE2018,Bansal_NAACL2019,Stoian_ICASSPP2020}.
To develop better methods, we can decouple pre-training into three problems: 1) What are the components of the ST model? 2) How to pre-train these components? 3) How to fine-tune the model?

We first highlight one research route called stacked encoding.
Several studies identify that the underlying issue of the single-encoder modeling is its weak ability to learn the acoustic and semantic features at the same time \cite{Liu_corr2020,Wang_acl2020,Wang_aaai2020,Xu_ACL2021}.
To this end, they decouple the encoding into an acoustic encoder and a semantic (or textual) encoder, where these two encoders are initialized by the ASR encoder and MT encoder respectively.

However, this results in the modality gap issue: the pre-trained MT encoder consumes the short sequence of word embedding but accepts the long sequence of acoustic representation during fine-tuning \cite{Liu_corr2020,Wang_aaai2020,Xu_ACL2021}.
Considering the representation gap and length gap, an adapter module is inserted between two encoders for better fine-tuning.
Specifically, \cite{Liu_corr2020} shrink the long acoustic sequence into a similar length of the transcription by removing the blank and merging the repeat tokens according to the CTC prediction.
\cite{Wang_aaai2020} share the weights of CTC and word embedding for the same representation space and pre-train the MT model with the noisy input.
Following the adaptive and informative principles, \cite{Xu_ACL2021} combine acoustic representation and soft representation by weighting the embedding matrix with the CTC distribution.

In addition, researchers explore better methods to pre-train the encoder, like supervised learning on semantic learning \cite{Wang_acl2020}, unsupervised masked acoustic modeling \cite{Chen_Corr2020}, and fused speech and text encoding \cite{Zheng_ICML2021}.
\cite{Alinejad_EMNLP2020} utilize adversarial learning to bridge the representation gap between the ASR encoder and MT decoder.
Rather than 
Also, \cite{Nguyen_ISCA2020,Wu_ISCA2020} use the self-supervised model like wav2vec \cite{Steffen_Interspeech2019} as the feature extractor, providing effective acoustic representation as the input.
% Overall, pre-training is an effective method for ST with scarce data.

\subsubsection{Multi-task Learning}
\input{section/multitask.tex}

\subsubsection{Knowledge Distillation}
\input{section/kd.tex}

% \subsubsection{Cross-lingual Transfer}
% e.g. multilingual ST
\subsubsection{Data Augmentation}
\input{section/data_aug.tex}


\subsubsection{Other, like meta-learning(1), adversarial(1)}

% \newpage

\section{How to Solve Modality Gap? }
\label{sec:modality_gap}
\subsection{Model Design}
\subsubsection{Acoustic-textual Representation}
\subsubsection{Transcription-Translation Optimization}
\subsection{Training Strategy}
\subsubsection{Self-Supervised Pretraining?}
\subsubsection{Curriculum Pretraining (1)}

% \section{Progress}
% \section{Model Modifications for End-to-end Speech Translation}
% \subsection{Bi-modal Inputs}
% Like Chimera, XSTNeT, fairseq's model
% \subsection{Two pass Encoders}
% Like LUT, SATE
% \subsection{Decoder Modifications}
% \subsubsection{Joint Decoding}
% like Baidu's interactive decoding
% \subsubsection{Non-autoregressive Decoding}
% like CTC from Lihongyi

% \subsection{Modeling Methods}
% \subsubsection{Encoder-decoder Approach}
% \subsubsubsection{LSTM/Transformer/Conformer}
% \subsubsection{Synchronization Mode}
% \subsubsubsection{Label/Frame Synchronization}
% \subsubsection{Acoustic-textual Representation}
% \subsubsubsection{Fusion/Disentanglement}
% \subsubsection{Disentanglement}
% \subsubsection{Transcription-Translation Optimization}
% \subsubsubsection{Independence/Dependence}
% \subsubsection{Dependence}
% \subsubsection{Acoustic-textual Alignment}
% Soft Alignment/Hard Alignment/Monotonic Alignment
% \subsubsection{...}



==> section/old_mlt.tex <==
% Multi-task learning~\cite{Caruana1997MultitaskL} helps the model training by adding additional training objectives. 
% Multi-task learning helps the model training by adding additional training objectives. 
% It is very effective for the end-to-end ST --- a complex task with insufficient supervised training data, because the additional loss terms
% 1) can be regarded as regularizations, which improve the model's robustness and avoid overfitting issues; and 
% 2) they can be used to leverage more (external) knowledge or information to the model by introducing other supervised data, such as transcription.


The idea of multi-task learning is to utilize related auxiliary tasks to enhance the target task. For ST, the auxiliary tasks are often ASR and MT. 
Some parameters of the target and auxiliary task models are shared. 
% Therefore, in most cases, multitask learning not only merely refers to the training method, but also includes the corresponding model framework.
Therefore, multitask learning typically refers to both the training method and the model framework.
In Section~\ref{sec:model} we presented some model structures other than the encoder-decoder model, which can be naturally used as multitask learning framework.
For example, the model with a decoupled decoder or a decoupled encoder can train ST and ASR tasks jointly~\cite{Anastasopoulos_NAACL2018,Inaguma_ASRU2021,Liu_AAAI2020,Le_COLING20202,Liu_corr2020,dong2021learning,Xu_ACL2021}, and the model with a two-stream encoder can train both ST and MT tasks~\cite{tang2021general,Ye_interspeech2021,tang2021improving}.
Note that when training multiple tasks, both sharing of modules for knowledge transfer and differentiation between tasks are necessary.
Simple yet effective, \cite{Ye_interspeech2021} added special token indicators to distinguish each task.
% \cite{indurthi2021task} designed a Task Characteristics Network (TCN) that produces a task embedding to modulate the parameters of the shared encoder-decoder. 

% \cite{Ye_interspeech2021} also used a similar structure and further extends it to accomplish ASR, ST, and MT tasks by a simple method of adding special token indicators. 
% \yr{add [icassp 2021][samsung] Task Aware Multi-Task Learning for Speech to Text Tasks
% ICLR review https://openreview.net/forum?id=kJVVgJ-yCq}

% Multi-task learning is also not limited to autoregressive generation tasks by sharing encoder or decoder modules. 
% Given that the speech input is usually an audio signal, which is much longer than a text sequence, this makes it difficult for the speech encoder to learn well. 
% Text transcription provides an alignment to the speech, which can bring more efficient information to enhance the speech encoder.
% Adding a Connectionist Temporal Classification (CTC) loss term after the speech encoder to predict the transcription can efficiently model such alignment.
% \cite{Liu_corr2020} proposed a shrinking mechanism based on CTC loss and integrated with multi-task learning.
% \cite{dong2021listen} introduced an additional pre-trained BERT model~\cite{devlin2019bert} to supervise the output of the speech encoder, in addition to CTC and translation loss, which enhances the semantic representation of the speech.

Multi-task learning can be naturally combined with pre-training. 
A unified encoder-decoder model is built to jointly pre-train ASR, MT, masked language model (MLM),  or even speech (re-)synthesis tasks using multilingual speech-text supervised data as well as large amounts of monolingual text and audio~\cite{ao2022speecht5,tang2022unified,bapna2022mslam,cheng2022mu}.
These multi-task pre-trained models can directly exploit more potential contextual knowledge in speech and text data and thus improve on many speech-related tasks, including but not limited to speech translation.


==> section/other_train.tex <==



% \noindent\textbf{Meta-learning}~
% Data Efficient Direct Speech-to-Text Translation with Modality Agnostic Meta-Learning

% \noindent\textbf{Adversarial learning}~
% End-to-End Speech Translation with Adversarial Training, WAST-2020
% Breaking the Data Barrier: Towards Robust Speech Translation via Adversarial Stability Training, IWSLT-2019

% \noindent\textbf{Regularization}~
% [AAAI2022] Regularizing End-to-End Speech Translation with Triangular Decomposition Agreement
% https://arxiv.org/pdf/2107.05782.pdf -- Cross-Attentive Regularization

==> section/s2st.tex <==
\subsection{Speech-to-speech Translation }
The task of speech to speech translation (S2ST) is to translate between acoustic features in different languages. In addition to the advantages over cascaded systems, end-to-end S2ST can be used for translation of languages without written systems, such as some dialects.

\paragraph{Metrics} 
% End-to-end evaluation of speech-to-speech translation is also a popular research topic recently. 
Evaluation for S2ST generally includes two aspects, the quality of the translation and the quality of the synthesized audio. In general, human evaluation is more reliable, which requires high labor costs.
% and the construction of end-to-end and reliable automatic evaluation indicators is also the need for rapid iterations of the model. 
The most popular automatic translation quality assessment method is ASR-BLEU, which needs to use an ASR model of the target language to recognize the transcribed text of the synthesized audio, and then calculate BLEU based on the transcribed text and the reference text (or the transcribed text of the reference audio). 
This process might introduce the recognition error of the ASR model. 
At the same time, the evaluation results depend on the used ASR model, and the numbers can not be directly compared between different research work. Recently, Meta proposes a text-independent speech translation evaluation metric, BLASER~\cite{chen2022blaser}, which can directly calculate translation scores for cross-language audios.

\paragraph{Model Structure} \cite{jia2019direct} firstly proves the possibility of accomplishing this process directly by a single model without separate text representation. 
Translatotron~\cite{jia2019direct} uses the encoder-decoder framework based on LSTM to learn the mapping between source spectrogram and target spectrogram, and adds two auxiliary tasks (including source phoneme recognition and target phoneme recognition) to relief the modeling burden.
Translatotron2~\cite{jia2022translatotron} consists of a speech encoder, a linguistic decoder, an acoustic synthesizer, and an attention module that connects the former three parts. This separate attention module can simultaneously provide acoustic information from the original speech and linguistic information of the target text, and can retain fine-grained non-linguistic information during the translation process.
Unit-based methods~\cite{lee2021direct,inaguma2022unity,li2022textless} usually first utilize a pre-trained acoustic model (such as Hubert~\cite{hsu2021hubert} ) for the Speech2Unit process, which translates the source speech into discrete units, and then use a unit-based vocoder to generate the target audio. Discrete units can decouple acoustic information and linguistic information to a certain extent, which can bring benefits to S2ST modeling.

\paragraph{Pseudo Labeling} End-to-end training requires relatively large data, and insufficient training data is one of the main challenges in current research in this field. The data augmentation method based on pseudo-labeling technology~\cite{jia2022leveraging,popuri2022enhanced,dong2022leveraging,nguyen2022improving} can effectively alleviate this challenge. The more common method is to use a machine translation engine to obtain pseudo-labeled translation labels, or use a speech synthesis engine to obtain pseudo-labeled audio labels, etc.
% \dqq{challenges} According to the previous literature's findings, direct S2ST model has a bias in the reconstruction of the input. For example, it will directly pronounce as the source speech without translation.


==> section/sist.tex <==
\subsection{Simultaneous Speech-to-text Translation}

% \subsubsection{Online Decoding algorithms}
Simultaneous speech translation (SiST) needs to balance translation quality and translation delay at the same time. On the one hand, for better user experience, SiST pursues lower latency, which requires starting translation as early as possible; on the other hand, in order to ensure the accuracy of translation, more context needs to be read in, which requires waiting as much as possible audio stream. In summary, the goal of SiST is to achieve the best translation accuracy while satisfying certain delay constraints.
\cite{ma2020simulmt} firstly defined the SiST task and adapted SiMT methods, wait-$k$~\cite{ma2018stacl} and monotonic multihead attention~\cite{ma2019monotonic}, to SiST.
% , and proposed fixed and flexible pre-decision, and fixed and flexible policies
\cite{ma2021streaming} proposed an augmented memory transformer encoder,  which can not only translate with partical audio input, but also handle very long or continuous audio. ~\cite{nguyen2021empirical} directly integrates a simultaneous decoding strategy into offline-trained ST models to do inference simultaneously.~\cite{papi2022does} also demonstrates that a offline-trained ST model can serve both the offline and online translation scenarios without any additional training or adaptation. 

\paragraph{Metrics} The evaluation of SiST includes translation quality and translation latency. The latency metrics are extended from simultaneous text translation (SiMT), including Average Lagging (AL), Average Proportion (AP), and Differentiable Average Lagging (DAL), calculated on speech sequence instead of word sequence. \dqq{add computation-aware metrics}

\paragraph{Model Structure} Current SiST work is mainly built on the attention-based encoder decoder framework, which requires unidirectional attention mask to keep training and testing consistent. 
\cite{liu2021cross} extends RNN-Transducer
% ~\cite{graves2012sequence}
into Cross Attention Augmented Transducer (CAAT) for SiST, which can jointly optimize the decoding policy and translation quality by considering all possible READ and WRITE action paths. CAAT also introduces a latency loss to directly optimize the translation delay.
\cite{xue2022large} proposes a Transformer transducer-based SiST model and experiments on a large scale 50,000 hours pseudo-labeled training set. 

\paragraph{Joint Training} \cite{weller2021streaming} develops a streaming model for joint ASR and SiST with a consecutive decoding based on a re-translation approach by interleaving both transcript and translation during generation.
\cite{chen2021direct} combines streaming ASR and SiST tasks with two separate, but synchronized decoders and uses the intermediate results of ASR to guide the decoding policy of SiST. 

\paragraph{Pre-decision} Since SiST predicts actions on continuous audio sequences, the fixed pre-decision strategy fixes the audio segments' duration of each READ action, which easily destroys the semantic integrity of audio information. Recently, there have been some works investigating adaptative segmentation strategies. 
SimulSpeech~\cite{ren2020simulspeech} proposes a speech segmenter, based on the connectionist temporal classification (CTC) criterion, to split the streaming speech in real time. To improve the translation performance, SimulSpeech introduces two-level knowledge distillation methods, attention-level and data-level.
RealTrans~\cite{zeng2021realtrans} uses a weighted-shrinking operation to map the length of speech feature sequence into text sequence's length and proposes a Wait-K-Stride-N strategy to allow local reranking during decoding.   
MoSST~\cite{dong2021learning} develops an efficient monotonic segmentation module based on Continuous Integrate-and-Fire (CIF) mechanism~\cite{dong2020cif} to make READ decisions at audio boundaries.

\paragraph{Policy}
The policy of SiST decides when to READ or WRITE. Most of existing work adapts the fixed wait-kk policy.
\cite{chang2022exploring} adapts CIF module to model adaptive policy, which makes WRITE decisions at each firing step.
~\cite{zaidi2021decision} proposes Decision Attentive Regularization (DAR) method to utilize the monotonic attention energies based on MMA model of SiMT to guide the policy of SiST. 


==> section/transfer_learning.tex <==
Transfer learning is a promising method that first pre-trains different components of the ST on external data, and then fine-tunes the model parameters on the small-scale ST data. 
% \cite{Zhuang_IEEE2021}.
The vanilla ST model adopts the encoder-decoder architecture, where a naive strategy initializes the encoder with the ASR model and the decoder with the MT model, and finally fine-tunes all the model parameters \cite{Berard_IEEE2018,Bansal_NAACL2019,Stoian_ICASSPP2020}.
To develop better methods, transfer learning can be decoupled into three problems: 1) What are the components of the ST model? 2) How to pre-train these components? 3) How to fine-tune the model?

As discussed in Section \ref{sec:model}, the model framework contains the vanilla encoder-decoder architecture and multiple variants.
The earlier work explores better pre-training methods to enhance the ability of the encoder in terms of semantic understanding, like supervised learning on semantic learning \cite{Wang_acl2020}, unsupervised masked acoustic modeling \cite{Chen_Corr2020}, and fused speech and text encoding \cite{Zheng_ICML2021}.
Instead of parameter initialization, the self-supervised model like Wav2vec \cite{Steffen_Interspeech2019} can act as the feature extractor \cite{Nguyen_ISCA2020,Wu_ISCA2020}, providing effective acoustic features as the input.
In addition, straightly fine-tuning the pre-trained ASR encoder and MT decoder may result in the representation gap.
\citet{Alinejad_EMNLP2020} close the representation of the ASR and MT encoders by adversarial learning, which makes the pre-trained components more compatible.

The recent work pays more attention on the multi-encoder designs.
Several studies identify that the underlying issue of the single encoder modeling is its weak ability to learn the acoustic and semantic features simultaneously \cite{Wang_acl2020,Wang_aaai2020,Xu_ACL2021}, which further leads to the ST model cannot inherit the full capability of the pre-trained models.
The decoupled encoder or two-stream encoder prevent this issue by initializing two encoders with the pre-trained ASR encoder and MT encoder respectively \cite{Wang_aaai2020,Xu_ACL2021}.
In addition, the self-supervised models like xxx can be used 

However, this results in the modality gap issue: the pre-trained MT encoder consumes the short sequence of word embedding but accepts the long sequence of acoustic representation during fine-tuning \cite{Liu_corr2020,Wang_aaai2020,Xu_ACL2021}.
Considering the representation gap and length gap, an adapter module is inserted between two encoders for better fine-tuning.
Specifically, \citet{Liu_corr2020} shrink the long acoustic sequence into a similar length of the transcription by removing the blank and merging the repeat tokens according to the CTC prediction.
\citet{Wang_aaai2020} share the weights of CTC and word embedding for the same representation space and pre-train the MT model with the noisy input.
Following the adaptive and informative principles, \citet{Xu_ACL2021} combine acoustic representation and soft representation by weighting the embedding matrix with the CTC distribution.

% In addition, researchers explore better methods to pre-train the encoder, like supervised learning on semantic learning \cite{Wang_acl2020}, unsupervised masked acoustic modeling \cite{Chen_Corr2020}, and fused speech and text encoding \cite{Zheng_ICML2021}.
% \cite{Alinejad_EMNLP2020} utilize adversarial learning to bridge the representation gap between the ASR encoder and MT decoder.
% Also, \cite{Nguyen_ISCA2020,Wu_ISCA2020} use the self-supervised model like wav2vec \cite{Steffen_Interspeech2019} as the feature extractor, providing effective acoustic representation as the input.
% Overall, pre-training is an effective method for ST with scarce data.


==> table/datasets.tex <==
\begin{table*}[!h]
    \centering
    \begin{tabular}{lp{3.5cm}p{4.1cm}l}
    \toprule
    \textbf{Dataset} & \textbf{Domain} & \textbf{Language} & \textbf{Avg. duration(h)} \\
    
    \midrule
    LibriTrans~\cite{kocabiyikoglu2018augmenting} & Audiobook & en$\rightarrow$ fr& 236\\
    IWSLT2018~\cite{niehues-etal-2018-iwslt}& TED &en$\rightarrow$ de&272 \\
    BSTC~\cite{zhang2021bstc}&Lecture & zh$\rightarrow$ en& 51\\
    TED-EnZh~\cite{liu2019end}&TED&en$\rightarrow$ zh& 542\\
    MuST-C~\cite{di2019must}&TED&en$\rightarrow$\{de, es, fr, it, nl, pt, ro, ru\} \yr{now v1.2?}& 452\\
    How2~\cite{sanabria2018how2} &Youtube&en$\rightarrow$ & 300 \\
    STC~\cite{shimizu2014collection} &?&en$\rightarrow$ jp& ? \\
    KIT~\cite{stuker2012kit} &Lecture& de$\rightarrow$ en& 37\\
    LibriVoxDeEn~\cite{beilharz2019librivoxdeen} &Audiobook&de$\rightarrow$ en& 100\\
    Europarl-ST~\cite{iranzo2020europarl} &Parliament&?& ?\\
   TED-EN-DE/FR/ZH/JP~\cite{liu2020synchronous} &TED&en$\rightarrow$\{de,fr,zh,jp\}& ?\\
   CoVoST~\cite{wang2020covost} &Common Voice&?& ?\\
    EPIC~\cite{bendazzoli2005approach}  & (Conference) Interpretation & \{it, en, sp\} & 6\\
    CIAIR~\cite{tohyama2004ciair} & (Monologue+Dialogue) Interpretation & en$\rightarrow$ ja & 180 \\
    SIC~\cite{doi2021large}& (News + Lecture) Interpretation & en$\rightarrow$ ja &22 \\
    EMIME proj.~\cite{wester2011emime}& Recording & en$\rightarrow$ de, en$\rightarrow$ fi, en$\rightarrow$ zh& 6\\
    SP2 Speech Corpus~\cite{sevcujski2016design}& Recording & \{en, fr, hu, se, ma\}$\rightarrow$ en & 0.15 \\
    Fisher~\cite{post2013improved} & Telephone Conversation & es$\rightarrow$ en & 127 \\
    LibriS2S~\cite{jeuris2022libris2s}  & Audiobook & en$\rightarrow$ de & 53 \\
    MaSS~\cite{boito2019mass} & Bible Reading & \{en, es, eu, fi, fr, hu, ro, ru\} & 21  \\
    VoxPopuli~\cite{wang2021voxpopuli}  & European Parliament & \{en, de, fr, es, pl, it, ro, hu, cs, nl, fi, sk, sl, lt, da\} &  82 \\
    CVSS~\cite{jia-etal-2022-cvss}  & Recording & \{ar, ca, cy, de, et, es, fa, fr, id, it, ja, lv, mn, nl, pt, ru, sl, sv, ta, tr, zh\}$\rightarrow$ en & 181 \\
    FLEURS~\cite{conneau2022fleurs} & Reading & \{...\}(102 languages) & 12 \\ 
    SpeechMatrix~\cite{duquenne2022speechmatrix} & European Parliament & \{cs, de, en, es, et, fi, fr, hr, hu, it, lt, nl, pl, pt, ro, sk, sl\} & 1537 \\
    % \corpus & Multi-Source & En\rightarrow\rightarrow Zh &10k \\
    \midrule
    \end{tabular}
    \caption{Comparison of existing speech translation datasets.}
    \label{tab:dataset}
\end{table*}

